Comparison of Attention-based Deep Learning Models for EEG Classification

Objective: To evaluate the impact on Electroencephalography (EEG) classification of different kinds of attention mechanisms in Deep Learning (DL) models. Methods: We compared three attention-enhanced DL models, the brand-new InstaGATs, an LSTM with attention and a CNN with attention. We used these models to classify normal and abnormal (i.e., artifactual or pathological) EEG patterns. Results: We achieved the state of the art in all classification problems, regardless the large variability of the datasets and the simple architecture of the attention-enhanced models. We could also prove that, depending on how the attention mechanism is applied and where the attention layer is located in the model, we can alternatively leverage the information contained in the time, frequency or space domain of the dataset. Conclusions: with this work, we shed light over the role of different attention mechanisms in the classification of normal and abnormal EEG patterns. Moreover, we discussed how they can exploit the intrinsic relationships in the temporal, frequency and spatial domains of our brain activity. Significance: Attention represents a promising strategy to evaluate the quality of the EEG information, and its relevance, in different real-world scenarios. Moreover, it can make it easier to parallelize the computation and, thus, to speed up the analysis of big electrophysiological (e.g., EEG) datasets.

==> baseline_models.tex <==
%%

%% GNN
\subsubsection {\gls{gnn}}
\hl{specify the form of the input for this model (how matrix r(t) is fed to the model.. column-wise, concatenation..)}
The first model we implemented share the same architecture with \glspl{instagats}, with the key difference that the first layer is a standard convolutional layer, as shown in Fig.~ \ref{fig:gnn}.
%
\textcolor{red}{Why here the standard convolution is applied? Is it the same operation like in CNN? I was sure that the convolution is performed in a neighbourhood of a given node, please explain}
This model is implemented in Python as \gls{instagats}.

\begin{figure*}[h]
	\centering
    \includegraphics[width=\hsize]{figures/gnn.png}
    \caption{Architecture of \gls{gnn}\textcolor{red}{what is the difference between figure representing GAT and this one} }\label{fig:gnn}
\end{figure*}



\subsubsection {\gls{lstm}}
The fourth model considered in this work is a standard \gls{lstm}, i.e., a specialized type of \gls{rnn} with a \hl{number $??$ of memory cells} to modulate the duration of the \gls{lstm}'s memory.
Indeed, the \gls{lstm} has the ability to remove or add information to the cell state through the gates. Gates are composed of a sigmoid neural network layer and a point-wise multiplication operation. Particularly, the sigmoid layer's output is a value in the range $[0, 1]$, describing the variation of the cell state.
%
\hl{specify the form of the input for this model (how matrix r(t) is fed to the model.. column-wise, concatenation..)}

\hl{This model is implemented in Python... }



\subsubsection {\gls{cnn}} %~\cite{Zhang_2019}}
The final model we considered is a standard \gls{cnn}.
\hl{specify the form of the input for this model (how matrix r(t) is fed to the model.. column-wise, concatenation..)}
Each unit in a layer receives inputs from a set of units in a small neighborhood in the previous layer, i.e., its \emph{receptive field}. Neurons learn to extract visual features that are subsequently combined in the next layer
to higher-order features~\cite{Lecun1999}.\textcolor{red}{We have only one convolutional layer - why?}
A convolutional layer extracts high-level features by multiplying a convolutional matrix, i.e., the \emph{kernel}, with the input data. The kernel of the convolution is the set of connection weights used by the units in the feature map.
The activation function used by neurons in the convolution layer is a $ReLU$ function, in line with most of the current literature.
A pooling Layer reduce the size of the feature map, decreasing the computational effort required through dimensional reduction, i.e., choosing the maximum in the output from the previous layer. At this step, the dominant features are extracted. % max pooling returns the maximum value of the slice of data covered by the kernel
To prevent overfitting, a dropout Layer~\cite{Srivastava2014} is added. % it also provides a way of approximately combining exponentially many different neural network architectures efficiently.
Finally, the classification task is operated by a \emph{dense layer}, namely a \gls{mlp}.
%
This final layer (similarly to the architecture based on attention mechanisms) allowed us to obtain, for each time frame \textcolor{red}{is it for one frame or concatenated frames from all channels?}, an embedded vector which corresponds to a graph of the \gls{cnnatt} model.\textcolor {red}{do we really consider a graph in this case?}
\GC{The embedding sequence can then be processed as input from the stacked \gls{lstm}?}
%
% It is worth to note that in our experiments we have also evaluated a \emph{CCN + dense} architecture. In this case, a CNN supplies the graph embedding for every time frame. The sequence of all embedding is then passed as input to the dense layer.
%
During training of all architectures, the number of epochs was fixed to $100$ and the cross entropy function was selected as loss function. The selected optimizer is an \emph{Adam Optimizer} with a learning rate of $10^{-5}$.


\begin{figure*}[h]
	\centering
    \includegraphics[width=\hsize]{figures/cnn.png}
    \caption{Architecture of \gls{cnn}.} \label{fig:cnn}
\end{figure*}

\textcolor{red}{In my opinion, this description looks very wordy. For publication it should be presented more formally !!!!}



